Perception Score, A Learned Metric for Open-ended Text Generation Evaluation

Automatic evaluation for open-ended natural language generation tasks remains a challenge. Existing metrics such as BLEU show a low correlation with human judgment. We propose a novel and powerful learning-based evaluation metric: Perception Score. The method measures the overall quality of the generation and scores holistically instead of only focusing on one evaluation criteria, such as word overlapping. Moreover, it also shows the amount of uncertainty about its evaluation result. By connecting the uncertainty, Perception Score gives a more accurate evaluation for the generation system. Perception Score provides state-of-the-art results on two conditional generation tasks and two unconditional generation tasks.

==> section/Discussion.tex <==
\section{Discussions}
\label{sec:discussion}

As we discussed in
the previous sections, a language model optimized only for perplexity generates coherent but bland
responses \citep{evaluation-survey}.

\subsection{Direction}

1. Ethetical Issues
2.  Potential direction
1 alternanate reference
2. human wirtten lexical difference
3. human created reference with better quality
4. human adversarial 
Perception shared linear share
uncertainty and sigmoid should be different
use (c) instead of c
show how to get P'
how to show robustness or adversarial attack.
